Wigner Distribution Deconvolution Adaptation for Live Ptychography Reconstruction

We propose a modification of Wigner Distribution Deconvolution (WDD) to support live processing ptychography. Live processing allows to reconstruct and display the specimen transfer function gradually while diffraction patterns are acquired. For this purpose we reformulate WDD and apply a dimensionality reduction technique that reduces memory consumption and increases processing speed. We show numerically that this approach maintains the reconstruction quality of specimen transfer functions as well as reduces computational complexity during acquisition processes. Although we only present the reconstruction for Scanning Transmission Electron Microscopy (STEM) datasets, in general, the live processing algorithm we present in this paper can be applied to real-time ptychographic reconstruction for different fields of application.

==> fig/Compress_Decompress/compress_decompress.tex <==
\pgfplotsset{every tick label/.append style={font=\LARGE}}
% This file was created by tikzplotlib v0.9.9.
\begin{tikzpicture}
\begin{groupplot}[group style={group size=3 by 1,horizontal sep=2em},width = 0.5*\textwidth, height=(0.5)*\textwidth]
\nextgroupplot[
colorbar horizontal,
colorbar style={xtick={0,0.95},xticklabels={0.0,$8.10^{5}$}, xticklabel style={/pgf/number format/fixed}},
colormap/viridis,
hide x axis,
hide y axis,
%point meta max=810487,
%point meta min=0.0,
point meta max=1,
point meta min=0,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=255.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=255.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=255.5, ymin=255.5, ymax=-0.5] {fig/Compress_Decompress/compress_decompress-000.png};

\nextgroupplot[
colorbar horizontal,
colorbar style={xtick={0.1,0.95},xticklabels={0.0, $1.10^{7}$}},
colormap/viridis,
hide x axis,
hide y axis,
point meta max=1,
point meta min=0,
%point meta max=14353222,
%point meta min=-556567.375,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=15.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=15.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=15.5, ymin=15.5, ymax=-0.5] {fig/Compress_Decompress/compress_decompress-001.png};

\nextgroupplot[
colorbar horizontal,
colorbar style={xtick={0.1,0.95},xticklabels={0.0, $6.10^{5}$}},
colormap/viridis,
hide x axis,
hide y axis,
point meta max=1,
point meta min=0,
%point meta max=620757.1875,
%point meta min=-376.438385009766,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=255.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=255.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=255.5, ymin=255.5, ymax=-0.5] {fig/Compress_Decompress/compress_decompress-002.png};
\end{groupplot}


\end{tikzpicture}


==> fig/Exp_Res/Exp_STO.tex <==
% This file was created by tikzplotlib v0.9.9.
\begin{tikzpicture}

\begin{groupplot}[group style={group size=5 by 1,horizontal sep=0.5em},width = 0.25*\textwidth, height=(0.25)*\textwidth]
\nextgroupplot[
colorbar horizontal,
colormap/blackwhite,
%hide x axis,
%hide y axis,
ticks = none,
title = (a),
ylabel = Scan y,
xlabel = Scan x,
point meta max=0.251606047153473,
point meta min=-0.261222332715988,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=127.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=127.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {fig/Exp_Res/Exp_STO-000.png};

\nextgroupplot[
colorbar horizontal,
colormap/blackwhite,
%hide x axis,
hide y axis,
ticks = none,
point meta max=0.333269238471985,
point meta min=-0.273211002349854,
title = (b),
xlabel = Scan x,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=127.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=127.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {fig/Exp_Res/Exp_STO-001.png};

\nextgroupplot[
colorbar horizontal,
colormap/blackwhite,
%hide x axis,
hide y axis,
ticks = none,
title = (c),
xlabel = Scan x,
point meta max=0.331693083047867,
point meta min=-0.285140573978424,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=127.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=127.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {fig/Exp_Res/Exp_STO-002.png};

\nextgroupplot[
colorbar horizontal,
colormap/blackwhite,
%hide x axis,
hide y axis,
title = (d),
ticks = none,
xlabel = Scan x,
point meta max=0.261677473783493,
point meta min=-0.184297353029251,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=127.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=127.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {fig/Exp_Res/Exp_STO-003.png};

\nextgroupplot[
colorbar horizontal,
colormap/blackwhite,
%hide x axis,
hide y axis,
ticks = none,
xlabel = Scan x,
title = (e),
point meta max=0.263222128152847,
point meta min=-0.165853321552277,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=127.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=127.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {fig/Exp_Res/Exp_STO-004.png};
\end{groupplot}
\end{tikzpicture}


==> fig/Exp_Res_SSB/Exp_STO_SSB.tex <==
% This file was created by tikzplotlib v0.9.9.
\begin{tikzpicture}
\begin{groupplot}[group style={group size=5 by 1,horizontal sep=0.5em},width = 0.25*\textwidth, height=(0.25)*\textwidth]
\nextgroupplot[
colorbar horizontal,
%colorbar style={xtick={-0.5,0,0.5},xticklabels={−0.5,0.0,0.5}},
colormap/blackwhite,
%hide x axis,
%hide y axis,
ticks = none,
title = (a),
ylabel = Scan y,
xlabel = Scan x,
point meta max=0.810894383465788,
point meta min=-0.798732729192162,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=127.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=127.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {fig/Exp_Res_SSB/Exp_STO_SSB-000.png};

\nextgroupplot[
colorbar horizontal,
colormap/blackwhite,
%hide x axis,
hide y axis,
ticks = none,
title = (b),
xlabel = Scan x,
point meta max=0.521422318986998,
point meta min=-0.319312126020433,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=127.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=127.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {fig/Exp_Res_SSB/Exp_STO_SSB-001.png};

\nextgroupplot[
colorbar horizontal,
%colorbar style={xtick={0,0.25},xticklabels={0.00,0.25}},
colormap/blackwhite,
%hide x axis,
hide y axis,
ticks = none,
title = (c),
xlabel = Scan x,
point meta max=0.360626965473703,
point meta min=-0.211943005959824,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=127.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=127.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {fig/Exp_Res_SSB/Exp_STO_SSB-002.png};

\nextgroupplot[
colorbar horizontal,
%colorbar style={xtick={0,0.25},xticklabels={0.00,0.25}},
colormap/blackwhite,
%hide x axis,
hide y axis,
title = (d),
ticks = none,
xlabel = Scan x,
point meta max=0.262921147093797,
point meta min=-0.158436343361057,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=127.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=127.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {fig/Exp_Res_SSB/Exp_STO_SSB-003.png};

\nextgroupplot[
colorbar horizontal,
colormap/blackwhite,
%hide x axis,
hide y axis,
ticks = none,
title = (e),
xlabel = Scan x,
point meta max=0.208665738235203,
point meta min=-0.106166752151338,
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=127.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=127.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=127.5, ymin=127.5, ymax=-0.5] {fig/Exp_Res_SSB/Exp_STO_SSB-004.png};
\end{groupplot}
\end{tikzpicture}


==> fig/Graphene/graphene.tex <==
\pgfplotsset{every tick label/.append style={font=\Large}}
% This file was created by tikzplotlib v0.9.9.
\begin{tikzpicture}
\begin{groupplot}[group style={group size=2 by 1 ,horizontal sep=8em},width = 0.5*\textwidth, height=(0.5)*\textwidth]
\nextgroupplot[
colorbar,
colorbar style={ylabel={},scaled y ticks=false,yticklabel style={/pgf/number format/fixed}},
colormap/blackwhite,
hide x axis,
hide y axis,
point meta max=0.0817124837924765,
point meta min=-0.0385599213157242,
tick align=outside,
tick pos=left,
title={\Large (a)},
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=64.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=63.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=64.5, ymin=63.5, ymax=-0.5] {fig/Graphene/graphene-000.png};

\nextgroupplot[
colorbar,
colorbar style={ylabel={},scaled y ticks=false,yticklabel style={/pgf/number format/fixed}},
colormap/blackwhite,
hide x axis,
hide y axis,
point meta max=0.0758501961827278,
point meta min=-0.0444900617003441,
tick align=outside,
tick pos=left,
title={\Large (b)},
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=64.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=63.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=64.5, ymin=63.5, ymax=-0.5] {fig/Graphene/graphene-001.png};
\end{groupplot}
\end{tikzpicture}


==> fig/Graphene_Dose/graphene_dose.tex <==
\pgfplotsset{every tick label/.append style={font=\LARGE}}
% This file was created by tikzplotlib v0.9.9.
\begin{tikzpicture}

\begin{groupplot}[group style={group size=4 by 2,horizontal sep=7em},width = 0.5*\textwidth, height=(0.5)*\textwidth]
\nextgroupplot[
colorbar,
colorbar style={ylabel={},scaled y ticks=false,yticklabel style={/pgf/number format/fixed}},
colormap/blackwhite,
hide x axis,
%hide y axis,
ylabel = \LARGE Pyptychostem,
ticks=none,
point meta max=0.818620385902381,
point meta min=-0.92146204970414,
tick align=outside,
tick pos=left,
title={\LARGE (a)},
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=64.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=63.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=64.5, ymin=63.5, ymax=-0.5] {fig/Graphene_Dose/graphene_dose-000.png};

\nextgroupplot[
colorbar,
colorbar style={ylabel={},scaled y ticks=false,yticklabel style={/pgf/number format/fixed}},
colormap/blackwhite,
hide x axis,
hide y axis,
point meta max=0.300468908197715,
point meta min=-0.271739084352959,
tick align=outside,
tick pos=left,
title={\LARGE (b)},
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=64.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=63.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=64.5, ymin=63.5, ymax=-0.5] {fig/Graphene_Dose/graphene_dose-001.png};

\nextgroupplot[
colorbar,
title = \LARGE (c),
colorbar style={ylabel={},scaled y ticks=false,yticklabel style={/pgf/number format/fixed}},
colormap/blackwhite,
hide x axis,
hide y axis,
point meta max=0.142447589832753,
point meta min=-0.0982114009253316,
tick align=outside,
tick pos=left, 
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=64.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=63.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=64.5, ymin=63.5, ymax=-0.5] {fig/Graphene_Dose/graphene_dose-002.png};

\nextgroupplot[
colorbar,
title =\LARGE (d),
colorbar style={ylabel={},scaled y ticks=false,yticklabel style={/pgf/number format/fixed}},
colormap/blackwhite,
hide x axis,
hide y axis,
point meta max=0.0965678188610724,
point meta min=-0.0569810105818717,
tick align=outside,
tick pos=left, 
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=64.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=63.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=64.5, ymin=63.5, ymax=-0.5] {fig/Graphene_Dose/graphene_dose-003.png};

\nextgroupplot[
colorbar,
colorbar style={ylabel={},scaled y ticks=false,yticklabel style={/pgf/number format/fixed}},
colormap/blackwhite,
ylabel = \LARGE Live \ac{WDD},
hide x axis,
%hide y axis,
ticks = none,
point meta max=0.750064551830292,
point meta min=-0.786512911319733,
tick align=outside,
tick pos=left,
%title={Dose 100.0},
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=64.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=63.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=64.5, ymin=63.5, ymax=-0.5] {fig/Graphene_Dose/graphene_dose-004.png};

\nextgroupplot[
colorbar,
colorbar style={ylabel={},scaled y ticks=false,yticklabel style={/pgf/number format/fixed}},colormap/blackwhite,
hide x axis,
hide y axis,
point meta max=0.228222250938416,
point meta min=-0.205519363284111,
tick align=outside,
tick pos=left,
%title={Dose 1000.0},
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=64.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=63.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=64.5, ymin=63.5, ymax=-0.5] {fig/Graphene_Dose/graphene_dose-005.png};

\nextgroupplot[
colorbar,
colorbar style={ylabel={},scaled y ticks=false,yticklabel style={/pgf/number format/fixed}},
colormap/blackwhite,
hide x axis,
hide y axis,
point meta max=0.108508415520191,
point meta min=-0.0837747529149055,
tick align=outside,
tick pos=left,
%title={Dose 10000.0},
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=64.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=63.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=64.5, ymin=63.5, ymax=-0.5] {fig/Graphene_Dose/graphene_dose-006.png};

\nextgroupplot[
colorbar,
colorbar style={ylabel={},scaled y ticks=false,yticklabel style={/pgf/number format/fixed}},colormap/blackwhite,
hide x axis,
hide y axis,
point meta max=0.084065780043602,
point meta min=-0.0580905973911285,
tick align=outside,
tick pos=left,
%title={Dose 100000.0},
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=64.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=63.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=64.5, ymin=63.5, ymax=-0.5] {fig/Graphene_Dose/graphene_dose-007.png};
\end{groupplot}
 

\end{tikzpicture}


==> fig/Line_Scan/Line_Scan_.tex <==
% This file was created by tikzplotlib v0.9.9.

\begin{tikzpicture}


\begin{groupplot}[group style={group size=1 by 2}]

\nextgroupplot[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Scan-X},
xmajorgrids,
xmin=0, xmax=65,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Radian},
ymajorgrids,
ymin=-0.0701272636651993, ymax=0.131961539387703,
ytick style={color=black},
yticklabel style={/pgf/number format/fixed},
ytick={-0.1,-0.05,0,0.05,0.1,0.15},
%yticklabels={−0.10,−0.05,0.00,0.05,0.10,0.15}
]
\addplot [thick, black]
table {%
0 -0.050489354878664
1 -0.0701272636651993
2 -0.0591630935668945
3 -0.0233903378248215
4 0.0107657378539443
5 0.0160889476537704
6 -0.00706898467615247
7 -0.0349986553192139
8 -0.0419206134974957
9 -0.0194121114909649
10 0.018635643646121
11 0.0478867813944817
12 0.049093421548605
13 0.0218143463134766
14 -0.0111008249223232
15 -0.0183865483850241
16 0.0145643223077059
17 0.0675057470798492
18 0.0944729670882225
19 0.0647531896829605
20 -0.00262001249939203
21 -0.0516179762780666
22 -0.04723896458745
23 -0.00953871477395296
24 0.0117596564814448
25 -0.00750179868191481
26 -0.0456231199204922
27 -0.0701223686337471
28 -0.0668219923973083
29 -0.039223812520504
30 0.000626950117293745
31 0.0408137924969196
32 0.0694612711668015
33 0.0708823204040527
34 0.0366325713694096
35 -0.0132839344441891
36 -0.0393619351089001
37 -0.0226130615919828
38 0.0201969165354967
39 0.05385971814394
40 0.0557367578148842
41 0.0329686664044857
42 0.00934133678674698
43 0.00254456326365471
44 0.0114810131490231
45 0.0179501846432686
46 0.0044644782319665
47 -0.0238600037992001
48 -0.0445106886327267
49 -0.0450799353420734
50 -0.0317003093659878
51 -0.0121648535132408
52 0.0197477471083403
53 0.0707080960273743
54 0.120839387178421
55 0.131961539387703
56 0.0892972350120544
57 0.0245720576494932
58 -0.00924817286431789
59 0.0130432471632957
60 0.0662525072693825
61 0.10173224657774
62 0.0933179557323456
63 0.0489187203347683
64 -0.00650979299098253
};
\addlegendentry{PyptychoSTEM dose}
\addplot [thick, blue]
table {%
0 -0.0528632439672947
1 -0.069170705974102
2 -0.0665184706449509
3 -0.050057977437973
4 -0.0316255390644073
5 -0.0250841081142426
6 -0.032770823687315
7 -0.0413588918745518
8 -0.0322659462690353
9 0.00228288397192955
10 0.0493202731013298
11 0.0815344601869583
12 0.0781081020832062
13 0.0427576750516891
14 0.00325387180782855
15 -0.0083293030038476
16 0.0196344740688801
17 0.0663103833794594
18 0.0922024846076965
19 0.0730596482753754
20 0.0210338551551104
21 -0.0280106980353594
22 -0.047875389456749
23 -0.0419566631317139
24 -0.0333595015108585
25 -0.0379544943571091
26 -0.0523885115981102
27 -0.0657985135912895
28 -0.0686876773834229
29 -0.0514933951199055
30 -0.00987929850816727
31 0.0428562834858894
32 0.0807832852005959
33 0.0827418565750122
34 0.0459533892571926
35 -0.00466906139627099
36 -0.0293214302510023
37 -0.00851418450474739
38 0.0413093827664852
39 0.0831924602389336
40 0.0884864181280136
41 0.0585117563605309
42 0.0195878427475691
43 -0.00266625406220555
44 -0.0030418261885643
45 0.00186086539179087
46 -0.00915047619491816
47 -0.0371321178972721
48 -0.0627537369728088
49 -0.0687066465616226
50 -0.0510708838701248
51 -0.0142836254090071
52 0.0359439440071583
53 0.089803546667099
54 0.126621082425117
55 0.12383184581995
56 0.0802871063351631
57 0.0278158634901047
58 0.00927735958248377
59 0.0393944606184959
60 0.0898346304893494
61 0.115365527570248
62 0.0942250266671181
63 0.0405887737870216
64 -0.0150826442986727
};
\addlegendentry{Live WDD dose}
\nextgroupplot[
legend cell align={left},
legend style={
  fill opacity=0.8,  
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
x grid style={white!69.0196078431373!black},
xlabel={Scan-X},
xmajorgrids,
xmin=0, xmax=65,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Radian},
ymajorgrids,
ymin=-0.0701272636651993, ymax=0.131961539387703,
ytick style={color=black},
ytick={-0.1,-0.05,0,0.05,0.1,0.15},
yticklabel style={/pgf/number format/fixed},
%yticklabels={−0.10,−0.05,0.00,0.05,0.10,0.15}
]
\addplot [thick, black]
table {%
0 -0.0107952244579792
1 -0.025405490770936
2 -0.0328737013041973
3 -0.0349596217274666
4 -0.0339399948716164
5 -0.0328682251274586
6 -0.0329361408948898
7 -0.029997119680047
8 -0.0158603470772505
9 0.0138185182586312
10 0.051137238740921
11 0.0768458470702171
12 0.0737725347280502
13 0.0425900556147099
14 0.00496662966907024
15 -0.0114887617528439
16 0.00533202709630132
17 0.0428106114268303
18 0.0735389515757561
19 0.0765591040253639
20 0.0514710731804371
21 0.0147901931777596
22 -0.0150690386071801
23 -0.029974227771163
24 -0.0329531133174896
25 -0.0314813405275345
26 -0.0310652200132608
27 -0.0325480215251446
28 -0.0319398939609528
29 -0.0220408942550421
30 0.00262703001499176
31 0.0384364910423756
32 0.0696074590086937
33 0.0767688676714897
34 0.053397860378027
35 0.0152284521609545
36 -0.00916341319680214
37 -0.000975164410192519
38 0.0334929972887039
39 0.0679069757461548
40 0.0773044526576996
41 0.056657001376152
42 0.0207317173480988
43 -0.0109343733638525
44 -0.0283026825636625
45 -0.0331605263054371
46 -0.0324194431304932
47 -0.0315709300339222
48 -0.0324040502309799
49 -0.0327450335025787
50 -0.0265142042189837
51 -0.00673845363780856
52 0.0269459933042526
53 0.062173068523407
54 0.0787076875567436
55 0.0645120069384575
56 0.0288767646998167
57 -0.00194532831665128
58 -0.0053327907808125
59 0.0198328327387571
60 0.0536485463380814
61 0.0722565352916718
62 0.0656585320830345
63 0.0409477837383747
64 0.0121774543076754
};
\addlegendentry{PyptychoSTEM infdose}
\addplot [thick, blue]
table {%
0 -0.0230483245104551
1 -0.0410829186439514
2 -0.0477836132049561
3 -0.0474081709980965
4 -0.0455981977283955
5 -0.0464794673025608
6 -0.0489686578512192
7 -0.0454659424722195
8 -0.0263981260359287
9 0.0107325939461589
10 0.0546918287873268
11 0.0842160731554031
12 0.0825211703777313
13 0.0515343025326729
14 0.0133854746818542
15 -0.0043489090166986
16 0.0110911251977086
17 0.0484004579484463
18 0.0805232971906662
19 0.0845455229282379
20 0.0570359490811825
21 0.0136248832568526
22 -0.0243319794535637
23 -0.0443605668842793
24 -0.0478102825582027
25 -0.0445267893373966
26 -0.0436563491821289
27 -0.0467938706278801
28 -0.0469485782086849
29 -0.033639095723629
30 -0.001631386927329
31 0.0416626781225204
32 0.0768215358257294
33 0.0843321606516838
34 0.0602517537772655
35 0.0222384557127953
36 -0.00146247737575322
37 0.00688269129022956
38 0.0410755015909672
39 0.075680322945118
40 0.085314929485321
41 0.0625927224755287
42 0.0205897521227598
43 -0.0192621555179358
44 -0.0424847267568111
45 -0.0481810308992863
46 -0.0450576394796371
47 -0.0428629070520401
48 -0.0452337525784969
49 -0.047257024794817
50 -0.0387088321149349
51 -0.0118908053264022
52 0.0298141110688448
53 0.0695049241185188
54 0.086027629673481
55 0.0702348276972771
56 0.0344405472278595
57 0.00525787472724915
58 0.00372365606017411
59 0.0297873970121145
60 0.0636575147509575
61 0.0816859006881714
62 0.0729216709733009
63 0.0431527756154537
64 0.00692250393331051
};
\addlegendentry{Live WDD infdose}
\end{groupplot}
\end{tikzpicture}




==> fig/Makefile <==
# Grace plots (xmgrace *.agr)
AGRFILES = $(wildcard *.agr)

# Fig drawings (xfig *.fig)
FIGFILES = $(wildcard *.fig)

TARGET = $(FIGFILES:%.fig=%.pdf) $(FIGFILES:%.fig=%.svg) $(AGRFILES:%.agr=%.pdf)

all: $(TARGET)

veryall: all

.PHONY: clean veryclean

%.eps:	%.fig
	fig2dev -L eps $< $@

%.pdf:	%.fig
	fig2dev -L pdf $< $@

%.svg:	%.fig
	fig2dev -L svg $< $@

%.png:	%.fig
	fig2dev -L png $< $@

%.pdf:	%.dot
	dot -Tpdf -o $@ $<

%.pdf:	%.gif
	convert $*.gif $*.pdf

%.eps:  %.agr
	gracebat -hdevice EPS $*.agr

%.pdf:  %.agr
	gracebat -hdevice EPS $*.agr && \
	epstopdf $*.eps && \
	rm -f $*.eps

clean:
	-rm -f *.bak

veryclean: clean
	-rm -f $(TARGET)


==> fig/Time_Space/Time_Increasing_Detector.tex <==
% This file was created by tikzplotlib v0.9.9.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
title={Computation Time (Increasing Detector Size)},
x grid style={white!69.0196078431373!black},
xlabel={Dimension},
xmajorgrids,
xmin=-0.15, xmax=3.15,
xtick style={color=black},
xtick={0,1,2,3},
xticklabel style={rotate=90.0},
xticklabels={
  {(128, 128, 128, 128)},
  {(128, 128, 256, 256)},
  {(128, 128, 512, 512)},
  {(128, 128, 1024, 1024)}
},
y grid style={white!69.0196078431373!black},
ylabel={Second},
ymajorgrids,
ymin=-31.8060517208651, ymax=695.225659335032,
ytick style={color=black}
]
\addplot [semithick, color0]
table {%
0 48.4365378008224
1 142.803748326376
2 628.170919927768
};
\addlegendentry{Min. PyptychoSTEM}
\addplot [semithick, color1]
table {%
0 48.9026154791936
1 148.907329213805
2 662.178763377946
};
\addlegendentry{Max. PyptychoSTEM}
\addplot [semithick, color2]
table {%
0 48.7635655221529
1 145.51568192523
2 631.714242130984
};
\addlegendentry{Med. PyptychoSTEM}
\addplot [semithick, color3]
table {%
0 1.24084423622116
1 2.18800726067275
2 11.16499918513
3 36.4011819907464
};
\addlegendentry{Min. LiveWDD}
\addplot [semithick, color4]
table {%
0 1.44986949488521
1 2.40706778224558
2 13.3134662616067
3 38.9858613256365
};
\addlegendentry{Max. LiveWDD}
\addplot [semithick, color5]
table {%
0 1.28532814211212
1 2.20637599169277
2 12.6033019011375
3 37.4177385710645
};
\addlegendentry{Med. LiveWDD}
\end{axis}

\end{tikzpicture}


==> fig/Time_Space/Time_Increasing_Scan.tex <==
% This file was created by tikzplotlib v0.9.9.
\begin{tikzpicture}

\definecolor{color0}{rgb}{0.12156862745098,0.466666666666667,0.705882352941177}
\definecolor{color1}{rgb}{1,0.498039215686275,0.0549019607843137}
\definecolor{color2}{rgb}{0.172549019607843,0.627450980392157,0.172549019607843}
\definecolor{color3}{rgb}{0.83921568627451,0.152941176470588,0.156862745098039}
\definecolor{color4}{rgb}{0.580392156862745,0.403921568627451,0.741176470588235}
\definecolor{color5}{rgb}{0.549019607843137,0.337254901960784,0.294117647058824}

\begin{axis}[
legend cell align={left},
legend style={
  fill opacity=0.8,
  draw opacity=1,
  text opacity=1,
  at={(0.03,0.97)},
  anchor=north west,
  draw=white!80!black
},
tick align=outside,
tick pos=left,
title={Computation Time (Increasing Scan Size)},
x grid style={white!69.0196078431373!black},
xlabel={Dimension},
xmajorgrids,
xmin=-0.15, xmax=3.15,
xtick style={color=black},
xtick={0,1,2,3},
xticklabel style={rotate=90.0},
xticklabels={
  {(128, 128, 128, 128)},
  {(256, 256, 128, 128)},
  {(512, 512, 128, 128)},
  {(1024, 1024, 128, 128)}
},
y grid style={white!69.0196078431373!black},
ylabel={Second},
ymajorgrids,
ymin=-151.738195939013, ymax=3213.80068791613,
ytick style={color=black}
]
\addplot [semithick, color0]
table {%
0 48.4365378008224
1 198.566349115688
2 820.951332927216
};
\addlegendentry{Min. PyptychoSTEM}
\addplot [semithick, color1]
table {%
0 48.9026154791936
1 200.651542238891
2 845.277078361716
};
\addlegendentry{Max. PyptychoSTEM}
\addplot [semithick, color2]
table {%
0 48.9026154791936
1 200.651542238891
2 845.277078361716
};
\addlegendentry{Med. PyptychoSTEM}
\addplot [semithick, color3]
table {%
0 1.24084423622116
1 14.7009206670336
2 228.391535849776
3 3038.61643695878
};
\addlegendentry{Min. LiveWDD}
\addplot [semithick, color4]
table {%
0 1.44986949488521
1 14.9085748037323
2 228.944406162947
3 3060.8216477409
};
\addlegendentry{Max. LiveWDD}
\addplot [semithick, color5]
table {%
0 1.28532814211212
1 14.8238621570636
2 228.593831763137
3 3048.47953498247
};
\addlegendentry{Med. LiveWDD}
\end{axis}

\end{tikzpicture}


==> fig/WSe2/wse2.tex <==
% This file was created by tikzplotlib v0.9.9.
\pgfplotsset{every tick label/.append style={font=\Large}}
\begin{tikzpicture}
\begin{groupplot}[group style={group size=2 by 1 ,horizontal sep=8em},width = 0.5*\textwidth, height=(0.5)*\textwidth]
\nextgroupplot[
colorbar,
colorbar style={ylabel={},scaled y ticks=false,yticklabel style={/pgf/number format/fixed}},
colormap/blackwhite,
hide x axis,
hide y axis,
point meta max=0.192112312229344,
point meta min=-0.0877391947777086,
tick align=outside,
tick pos=left,
title={\Large (a)},
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=144.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=125.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=144.5, ymin=125.5, ymax=-0.5] {fig/WSe2/wse2-000.png};
\nextgroupplot[
colorbar,
colorbar style={ylabel={},scaled y ticks=false,yticklabel style={/pgf/number format/fixed}},
colormap/blackwhite,
hide x axis,
hide y axis,
point meta max=0.185249924659729,
point meta min=-0.0717248097062111,
tick align=outside,
tick pos=left,
title={\Large (b)},
x grid style={white!69.0196078431373!black},
xmin=-0.5, xmax=144.5,
xtick style={color=black},
y dir=reverse,
y grid style={white!69.0196078431373!black},
ymin=-0.5, ymax=125.5,
ytick style={color=black}
]
\addplot graphics [includegraphics cmd=\pgfimage,xmin=-0.5, xmax=144.5, ymin=125.5, ymax=-0.5] {fig/WSe2/wse2-001.png};
\end{groupplot}
\end{tikzpicture}

